Online On-Demand Multi-Robot Coverage Path Planning

We present an online centralized path planning algorithm to cover a large, complex, unknown workspace with multiple homogeneous mobile robots. Our algorithm is horizon-based, synchronous, and on-demand. The recently proposed horizon-based synchronous algorithms compute all the robots' paths in each horizon, significantly increasing the computation burden in large workspaces with many robots. As a remedy, we propose an algorithm that computes the paths for a subset of robots that have traversed previously computed paths entirely (thus on-demand) and reuses the remaining paths for the other robots. We formally prove that the algorithm guarantees complete coverage of the unknown workspace. Experimental results on several standard benchmark workspaces show that our algorithm scales to hundreds of robots in large complex workspaces and consistently beats a state-of-the-art online centralized multi-robot coverage path planning algorithm in terms of the time needed to achieve complete coverage. For its validation, we perform ROS+Gazebo simulations in five 2D grid benchmark workspaces with 10 Quadcopters and 10 TurtleBots, respectively. Also, to demonstrate its practical feasibility, we conduct one indoor experiment with two real TurtleBot2 robots and one outdoor experiment with three real Quadcopters.

==> 2023_09_16/1_abstract.tex <==
We present an online centralized path planning algorithm to cover a large, complex, unknown workspace with multiple homogeneous mobile robots. 
Our algorithm is horizon-based, synchronous, and on-demand. 
The recently proposed horizon-based synchronous algorithms compute the paths for all the robots in each horizon, significantly increasing the computation burden in large workspaces with many robots. 
As a remedy, we propose an algorithm that computes the paths for a subset of robots that have traversed previously computed paths entirely (thus on-demand) and reuses the previously computed paths for the other robots. 
We formally prove that the algorithm guarantees the complete coverage of the unknown workspace. 
Experimental results show that our algorithm scales to hundreds of robots in large workspaces and consistently outperforms a state-of-the-art online multi-robot centralized coverage path planning algorithm.
We also perform ROS+Gazebo simulations in five $2$D grid benchmark workspaces with $10$ Quadcopters and one outdoor experiment with two real Quadcopters to establish its practical feasibility. 
\is{The last line needs to be updated.}

==> 2023_09_16/2_introduction.tex <==
%====================================================================================================
\section{Introduction}
\label{sec-intro}


Coverage Path Planning (CPP) deals with finding conflict-free routes for a fleet of robots to make them completely visit the obstacle-free regions of a given workspace to accomplish some designated task. 
It has numerous applications in indoor environments, e.g.,  vacuum cleaning \cite{DBLP:conf/icra/BormannJHH18, DBLP:conf/icra/VandermeulenGK19}, industrial inspection \cite{DBLP:conf/iros/JingPGRLS17}, etc.,  as well as in outdoor environments, e.g.\longversion{, road sweeping \cite{DBLP:conf/icra/EngelsonsTH22}, lawn mowing \cite{DBLP:conf/iros/SchirmerBS17}}, precision farming~\cite{DBLP:journals/jfr/BarrientosCCMRSV11}\longversion{, \cite{DBLP:conf/atal/LuoNKS19}}, surveying~\cite{DBLP:conf/icra/KarapetyanMLLOR18}\longversion{, \cite{DBLP:conf/icra/AgarwalA20}}, search and rescue operations \longversion{\cite{DBLP:conf/iros/LewisEBRO17}, }\cite{cabreira2019survey}, \longversion{demining a battlefield~\cite{DBLP:conf/icra/DogruM19}, }etc. 
A CPP algorithm, often called a Coverage Planner (CP), is said to be \textit{complete} if it guarantees coverage of the entire obstacle-free region. 
Though a \textit{single} robot is enough to achieve complete coverage of a small environment (e.g., \cite{DBLP:conf/iros/BouzidBS17, DBLP:conf/iros/KleinerBKPM17, DBLP:conf/atal/SharmaDK19}\longversion{, \cite{DBLP:conf/icra/WeiI18, DBLP:conf/icra/CoombesCL19}}, \cite{DBLP:conf/iros/ChenTKV19, DBLP:conf/icra/DharmadhikariDS20}\longversion{, \cite{DBLP:conf/icra/ZhuYLSJM21}}), 
\textit{multiple} robots (e.g., \cite{DBLP:journals/ras/GalceranC13, DBLP:conf/icra/ModaresGMD17, DBLP:conf/iros/KarapetyanBMTR17}\longversion{, \cite{DBLP:conf/atal/SalarisRA20, DBLP:conf/icra/AgarwalA20}}, \cite{DBLP:conf/icra/VandermeulenGK19, DBLP:conf/iros/HardouinMMMM20, DBLP:conf/icra/TangSZ21, DBLP:conf/icra/CollinsGEDDC21}) facilitate complete coverage of a large environment more quickly. 
However, the design complexity of the CP grows significantly to exploit the benefit of having multiple robots. 

% For several CPP applications, the obstacle map of the workspace is not known a priori. 
% Thus, the \textit{offline} CPs (e.g., \longversion{\cite{DBLP:conf/icra/HazonK05, DBLP:conf/iros/ZhengJKK05, DBLP:conf/atal/RivaA17}, }\cite{DBLP:conf/iros/KleinerBKPM17, DBLP:conf/icra/BormannJHH18}\longversion{, \cite{DBLP:conf/atal/SalarisRA20, DBLP:conf/icra/CaoZTC20, DBLP:conf/iros/RamachandranZPS20, DBLP:conf/icra/SongYQSLL0022}}) that require the obstacle map beforehand are not useful here.
% Rather, we need an \textit{online} CP (e.g., \cite{DBLP:conf/agents/Yamauchi98}\longversion{, \cite{DBLP:journals/ijrr/HowardPS06}}, \cite{DBLP:conf/icra/BircherKAOS16}\longversion{, \cite{DBLP:conf/mesas/MannucciNP17, DBLP:conf/atal/JensenG18}}, \cite{DBLP:conf/iccps/DasS18, DBLP:conf/icra/OzdemirGKHG19, DBLP:conf/iros/HardouinMMMM20}\longversion{, \cite{DBLP:conf/iros/DattaA21}}) that runs through multiple rounds to cover the entire workspace gradually. 
% In each round, the robots explore some unexplored regions, and the CP subsequently finds the subpaths to cover the explored obstacle-free regions not covered so far. 

For many CPP applications, the workspace's obstacle map is unknown initially. 
So, the \textit{offline} CPs (e.g., \longversion{\cite{DBLP:conf/icra/HazonK05, DBLP:conf/iros/ZhengJKK05, DBLP:conf/atal/RivaA17}, }\cite{DBLP:conf/iros/KleinerBKPM17, DBLP:conf/icra/BormannJHH18}\longversion{, \cite{DBLP:conf/atal/SalarisRA20, DBLP:conf/icra/CaoZTC20, DBLP:conf/iros/RamachandranZPS20, DBLP:conf/icra/SongYQSLL0022}}) that require the obstacle map beforehand are not applicable here.
Instead, we need an \textit{online} CP (e.g., \cite{DBLP:conf/agents/Yamauchi98}\longversion{, \cite{DBLP:journals/ijrr/HowardPS06}}, \cite{DBLP:conf/icra/BircherKAOS16}\longversion{, \cite{DBLP:conf/mesas/MannucciNP17, DBLP:conf/atal/JensenG18}}, \cite{DBLP:conf/iccps/DasS18, DBLP:conf/icra/OzdemirGKHG19, DBLP:conf/iros/HardouinMMMM20}\longversion{, \cite{DBLP:conf/iros/DattaA21}}) that runs through multiple rounds to cover the entire workspace gradually. 
In each round, the robots explore some unexplored regions using attached sensors, and the CP subsequently finds their subpaths to cover the explored obstacle-free regions not covered so far, a.k.a. \textit{goals}. 

Based on where the CP runs, we can classify it as either \textit{centralized} or \textit{distributed}. 
A centralized CP (e.g., \cite{DBLP:conf/icra/GabrielyR01, DBLP:conf/agents/Yamauchi98, DBLP:conf/icra/BircherKAOS16}, \longversion{\cite{DBLP:conf/atal/RivaA17}, }\cite{DBLP:conf/iros/KleinerBKPM17, DBLP:conf/iccps/DasS18, DBLP:conf/atal/SharmaDK19}\longversion{, \cite{DBLP:conf/atal/SalarisRA20, DBLP:conf/icra/LiRS21}}, \cite{DBLP:conf/iros/MitraS22}) runs at a server and is responsible for finding all the paths alone. 
In contrast, a distributed CP (e.g., \longversion{\cite{butler2001complete}, }\cite{DBLP:conf/icra/HazonMK06}\longversion{, \cite{DBLP:journals/amai/RekleitisNRC08, DBLP:conf/ijcai/JensenG13, DBLP:conf/dars/HungerfordDG14}}, \cite{DBLP:journals/apin/VietDCC15}\longversion{, \cite{DBLP:conf/icra/SiligardiPKMGBS19, DBLP:journals/arobots/SongG20, DBLP:conf/iros/HassanML20}}) runs at every robot as a local instance, and these local instances \textit{collaborate} among themselves to find individual paths. 
The distributed CPs are computationally faster as they deal with only the local state spaces. 
However, \st{the paths generated by these methods are}\dm{they find} highly inefficient\dm{ paths} due to the lack of global knowledge about the state space. 
Despite having high computation time, the centralized CPs can provide a shorter 
% mission 
coverage 
completion time as they can find highly efficient paths by exploiting the global state space. 
The recently proposed online multi-robot centralized coverage planner \FnGAMRCPP~\cite{DBLP:conf/iros/MitraS22}\dm{, which is based on a \textit{receding horizon} strategy (e.g., \cite{DBLP:conf/icra/BircherKAOS16, DBLP:conf/iccps/DasS18}),} demonstrates this capability, thereby outperforming the state-of-the-art online multi-robot distributed coverage planner $\mathtt{BoB}$~\cite{DBLP:journals/apin/VietDCC15}. 

% This paper aims to develop a highly scalable online multi-robot centralized CP that guarantees complete workspace coverage.


% This paper aims to develop a highly scalable online multi-robot centralized CP that ensures complete coverage. 
% \st{Due to the scalability potential of \FnGAMRCPP, }\dm{\FnGAMRCPP has tremendous scalability potential because it is based on a \textit{receding horizon} strategy (e.g., \cite{DBLP:conf/icra/BircherKAOS16, DBLP:conf/iccps/DasS18}). So, }
% we \st{study the possibility of improving}\dm{aim to improve} it so that the new CP scales for hundreds of robots in large workspaces. 
% In each \textit{horizon} of \FnGAMRCPP, the CP plans for all the robots \textit{synchronously} (i.e., at the same time) using the currently available information about the workspace to ensure the coverage of at least one goal. 
% These generated paths may have different lengths. 
% A naive approach considered by \FnGAMRCPPMax \cite{DBLP:conf/iros/MitraS22}, a variant of \FnGAMRCPP, to decide the \textit{horizon length} is to set it as the \textit{maximum} length of the generated paths. 
% But, this approach has two major drawbacks. 
% First, the robots reaching their goals earlier must wait for the robots with the longest paths to reach their goals. 
% Second, the CP misses the opportunity to plan based on the accumulated intermediate information, which might lead to a better robot-goal assignment. 
% To address these two issues, \FnGAMRCPP advocates using the \textit{minimum} length of the generated paths to be the horizon length and shows that this approach significantly outperforms the former. 
% \dm{Could we get any better word in place of 'improve'? It may demean the contribution.}
% \is{What about removing the whole paragraph? What are we going to lose?}

A major bottleneck of \FnGAMRCPP is that it generates the paths for \textit{all} the robots \textit{synchronously} (i.e., at the same time) in each \textit{horizon} (like \cite{DBLP:conf/iccps/DasS18}), which prevents it from scaling for hundreds of robots in large workspaces. 
Furthermore, \FnGAMRCPP decides the horizon length based on the \textit{minimum} path length and \textit{discards} the remaining paths for the robots with longer paths. 
Finding a better goal assignment for those robots in the next horizon is possible, but discarding the already generated paths leads to considerable computational wastage. 
In this paper, we propose an alternative approach where, like \FnGAMRCPP, the CP decides the horizon length based on the minimum path length but \textit{keeps} the remaining paths for the robots with longer paths for traversal in the subsequent horizons. 
Thus, in a horizon, our proposed CP has to synchronously generate the paths for only those robots for which no remaining path is available
% \st{ 
(called the \textit{participant robots})
% }\dm{Let us not introduce this term here as they are nicely explained later in Section 3.}
, hence \textit{on-demand}. 
%\dm{So, it is computationally efficient. }
However, this new on-demand approach brings the additional challenge of computing the new paths under the constraint of the remaining paths for some robots. 
Our CP tackles this challenge in a sound %\st{and efficient }
manner. 
%\is{added the following line.}
Though the proposed \st{method may }\dm{approach }miss\dm{es} the opportunity to find more optimal paths for the \textit{non-participant robots} in a horizon, the computation load in each horizon reduces significantly, which in turn leads to a 
\st{noticeable improvement in the overall mission time for large workspaces and hundreds of robots. }
\dm{faster coverage completion of large workspaces with hundreds of robots, promising \textit{scalability}. }
% \dm{The last line may give a wrong impression that the generated paths are more efficient than those generated by GAMRCPP. OnDemCPP is efficient overall because it is only computationally efficient, not in path length (though sound in collision-free path generation). This is what we want to convey. One of the reviewers might have noted this term and questioned it. }

We formally prove that the proposed CP is guaranteed to achieve complete coverage. 
To evaluate its performance, we consider eight large $2$D grid-based benchmark workspaces of varying size and obstacle density and two types of robots, TurtleBot\longversion{ \cite{key_turtlebot}}, which is a ground robot, and Quadcopter, which is an aerial robot, for their coverage. 
We vary the number of robots from $128$ to $512$ and choose \textit{mission time} as the comparison metric, which is the time required to attain complete coverage. 
We compare our proposed CP with \FnGAMRCPP and show that it outperforms \FnGAMRCPP consistently for all instances involving large numbers of robots. We further demonstrate the practical feasibility of our algorithm through ROS+Gazebo simulations and real experiments. 

==> 2023_09_16/5_solution.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{On-Demand CPP Framework}
\label{sec:asyn_cpp}


This section presents the proposed centralized horizon-based online multi-robot on-demand CPP approach for complete coverage of an unknown workspace whose size and boundary are only known to the CP and the mobile robots. 

Due to the limited range of the fitted  rangefinders, each robot gets a \textit{partial} view of the unknown workspace, called the \textit{local view}. 
Initially, all the robots share their initial local views with the CP by sending \textit{requests} for paths. 
The CP then fuses these local views to get the \textit{global view} of the workspace. 
Based on the global view, it attempts to generate collision-free paths for the robots, possibly of different lengths. 
The robots with \textit{non-zero-length} paths are said to be \textit{active}, while the rest are \textit{inactive}. 
Next, the CP determines the horizon length as the minimum path length of the active robots. 
Subsequently, it makes the paths of the active robots of length equal to that horizon length. 
If any active robot's path length exceeds the horizon length, the CP stores the remaining part for future horizons. 
Finally, the CP provides these equal-length paths to respective active robots by sending \textit{responses}. 
As the CP has failed to find paths for the inactive robots in the current horizon, it considers them again in the next horizon. 
However, the active robots follow their received paths synchronously and update their local views accordingly. 
Upon finishing the execution of their current paths, they share their updated local views with the CP again. 
% In the next horizon, after updating the global view, the CP attempts to generate paths for the previous horizon's inactive robots and active robots who have completed following their paths. 
In the next horizon, after updating the global view, the CP attempts to generate paths for the previous horizon's inactive robots and active robots who have completed following their last planned paths. 
% \is{These robots are called \textit{participants}.}
In other words, the CP generates paths for only those robots with no remaining path, called the \textit{participants}. 
% Note that the robots with remaining paths computed in the previous horizon become the \textit{non-participants} (inherently active) in the next horizon. 
Note that the robots with remaining paths computed in the previous horizon become the \textit{non-participants} (inherently active) in the current horizon. 
Moreover, the CP does not alter the non-participants' remaining paths while generating the participants' paths in the current horizon. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.35]{figures/pdf/asyncpp.pdf}
    \caption{Overview of on-demand CPP}
    \label{fig:asyncpp}
\end{figure}

\begin{example}
\label{ex:update_gv}
In Figure~\ref{fig:asyncpp}, we show a schematic diagram of the on-demand CPP approach for three robots in an arbitrary workspace. 
In horizon $1$, the CP finds paths of lengths $0, 2$, and $3$ for the participants $r^1, r^2$, and $r^3$, respectively. 
Observe that only $r^2$ and $r^3$ are active. 
As the horizon length turns out to be $2$, the CP stores the remaining part of $r^3$'s path. 
Now, $r^2$ and $r^3$ follow their equal-length paths while $r^1$ waits. 
In horizon $2$, however, the CP finds paths only for $r^1$ and $r^2$ (notice the new colors) as non-participant $r^3$ already has its remaining path (notice the same color) found in horizon $1$. 
\end{example}


\input{5a_ds.tex}
\input{5b_overall.tex}
\input{5c_horizon.tex}
\shortversion
{
\input{5d_participants_short.tex}
}
\longversion
{
\input{5d_participants.tex}
}

==> 2023_09_16/5c_horizon.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Coverage Path Planning in the Current Horizon}
\label{subsec:cpp_horizon}

Here we describe the rest of Algorithm \ref{algo:ondemcpp}. 
Recall that the CP has already assigned the goals $\widetilde{W_g}$ to the non-participants in some past horizons. 
In \FnOnDemCPPHor (lines \shortversion{23-36}\longversion{37-50}), first, the CP checks whether there are \textit{unassigned} goals, i.e., $W_g \setminus \widetilde{W_g}$ left in the workspace (line \shortversion{25}\longversion{39}). 
If so, it attempts to generate the collision-free paths $\Sigma' = \{\sigma'^i\ |\ i \in I_{par}\}$ for the participants $I_{par}$ to visit some unassigned goals while keeping the remaining paths $\Sigma_{rem}$ of the non-participants $[R] \setminus I_{par}$ (hereafter denoted by $\overline{I_{par}}$) \textbf{intact} (line \shortversion{26}\longversion{40}). 
We defer the description of \FnCPPForPar to Section~\ref{subsec:cpp_for_par}. 
Otherwise, the CP cannot plan for the participants. 
Thereby, it \textit{skips} replanning the participants in the current horizon. 
Still, if there are non-participants (line \shortversion{27}\longversion{41}), they can proceed toward their assigned goals in the current horizon while the participants remain inactive. 
To signify this, the CP assigns the current states of the participants to their paths $\Sigma'$ (lines \shortversion{28-30}\longversion{42-44}). 
\shortversion{\dm{Please see Example 4 in \cite{DBLP:conf/arxiv/MitraS23}, where we show such a scenario. }}
Note that when both the criteria, viz all the robots are participants, and there are no unassigned goals get fulfilled (lines \shortversion{31-32}\longversion{45-46}), it means complete coverage \shortversion{(please refer to Section \ref{sec:theoretical_analysis})}\longversion{(established in Theorem \ref{theorem:asyncpp_complete_coverage})}. 
Next, the CP combines $\Sigma'$ with $\Sigma_{rem}$ into $\Sigma'_{all} = \{\sigma'^i_{all} | i \in [R]\}$, where %\st{\mbox{$\sigma'^i_{all} = (i \in I_{par})\ ?\ \sigma'^i:\sigma^i_{rem}$}. }
%\is{Write in sentence. A reviewer could not understand it.}
%
%\dm{
$$
\sigma'^i_{all}=
    \begin{cases}
        \sigma'^i, & \text{if $i \in I_{par}$}\\
        \sigma^i_{rem}, & \text{otherwise}.
    \end{cases}
$$
%}

So, $\sigma'^i_{all}$ contains the collision-free path $\sigma'^i$ if $r^i$ is a participant, otherwise contains the remaining path $\sigma^i_{rem}$ of the non-participant $r^i$. 
Notice that $\Sigma'_{all}$ contains the collision-free paths for all the robots (line \shortversion{33}\longversion{47}). 
A robot $r^i$ is said to be active in the current horizon if its path length is non-zero, i.e., $|\sigma'^i_{all}| > 0$. 
Otherwise, $r^i$ is said to be inactive. 
\is{Here, it looks like we are saying the same thing multiple times.}
In the penultimate step, the CP determines the length of the current horizon (line \shortversion{34}\longversion{48}) as the minimum path length of the active robots, i.e., $\lambda = \min_{i \in [R]} \{|\sigma'^i_{all}| > 0\}$. 
Finally, it returns $\lambda$-length paths $\Sigma$ only for the active robots (lines \shortversion{35-36}\longversion{49-50}). 
This way, the CP ensures that at least one active robot (participant or non-participant) reaches its goal in the current horizon. 

% \input{algorithms/ondemcpp_hor}

In $\mathtt{get\_equal\_length\_paths}$ (lines \shortversion{37-56}\longversion{51-70}), after re-initialization of some of the data structures (lines \shortversion{38-39}\longversion{52-53}), the CP examines the paths $\Sigma'_{all}$ in a \textbf{for} loop (lines \shortversion{40-55}\longversion{54-69}) to determine which robots are active (lines \shortversion{41-49}\longversion{55-63}), and which are not (lines \shortversion{50-54}\longversion{64-68}). 
If $r^i$ is active, first, the CP increments $N_{act}$ by $1$ (line \shortversion{42}\longversion{56}). 
Then, the CP splits its path $\sigma'^i_{all}$ into two parts $\sigma^i$ and $\sigma^i_{rem}$ of lengths $\lambda$ and $|\sigma'^i_{all}| - \lambda$, respectively (line \shortversion{43}\longversion{57}). 
Active $r^i$ traverses the former part $\sigma^i$, containing $s^i_0 \ldots s^i_{\lambda}$, in the current horizon (line \shortversion{44}\longversion{58}) and the later part (if any), containing $s^i_{\lambda} \ldots s^i_{|\sigma'^i_{all}|}$, in the future horizons (line \shortversion{55}\longversion{69}). 
If it has the remaining path $\sigma^i_{rem}$, its goal location $\mathcal{L}(s^i_{|\sigma'^i_{all}|})$ gets added to $\widetilde{W_g}$ (lines \shortversion{45-46}\longversion{59-60}), signifying that this goal remains reserved for $r^i$. 
Otherwise, $\sigma^i_{rem}$ is set to $\mathsf{NULL}$ (lines \shortversion{47-48}\longversion{61-62} and \shortversion{55}\longversion{69}), indicating the absence of the remaining path for $r^i$, thereby enabling $r^i$ to become a participant in the next horizon. 
In contrast, if $r^i$ is inactive (lines \shortversion{50-54}\longversion{64-68}), the CP adds $r^i$'s ID $\{i\}$ and its start state $s^i_0$ into $I^{inact}_{par}$ and $S^{inact}$, respectively (lines \shortversion{51-52}\longversion{65-66}), as it would reattempt to find $r^i$'s path in the next horizon. 
The CP also sets $\sigma^i_{rem}$ to $\mathsf{NULL}$ (lines \shortversion{53}\longversion{67} and \shortversion{55}\longversion{69}). 
Note that the CP also generates the full path for the active robots (line \shortversion{49}\longversion{63}) and the inactive robots (line \shortversion{54}\longversion{68}), where $\mathtt{dummy\_paths}$ generates a path of length $\lambda$ containing only the current state. 
The CP sends no path to an inactive robot in the current horizon (lines \shortversion{20-22}\longversion{34-36}). 
So, the active robots of the current horizon send requests in the next horizon (lines \shortversion{42}\longversion{56} and 11-12). 

\longversion
{
\begin{example}
\label{ex:skip_plan_par}
In Figure \ref{fig:skip_replan_par}, we show an example (continuation of Example \ref{ex:update_gv}) where the CP skips planning for a participant due to the unavailability of an unassigned goal. 
In horizon $1$, both the robots $r^1$ and $r^2$ participate, and the CP finds their collision-free paths $\sigma'^1$ and $\sigma'^2$ of lengths $2$ and $1$, respectively. 
Note that both robots are active. 
As the horizon length ($\lambda$) is found to be $1$, the CP reserves $r^1$'s goal into $\widetilde{W_g}$, and sets its remaining path $\sigma^1_{rem}$ accordingly. 
Each robot follows its $1$-length path and sends the updated local view to the CP. 
In horizon $2$, though the CP receives $2$ requests, only $r^2$ participates. 
As no unassigned goal exists (i.e., $W_g \setminus \widetilde{W_g} = \emptyset$), the CP fails to find any path for $r^2$. 
So, $r^2$ becomes inactive, and the CP adds its ID into $I^{inact}_{par}$ and state into $S^{inact}$ as it would reattempt in horizon $3$. 
Now, only $r^1$ (non-participant) is active. 
As $\lambda$ is found to be $1$, $r^1$ visits its reserved goal, which the CP removes from $\widetilde{W_g}$ and resets $\sigma^1_{rem}$. 
Notice that in horizon $3$, the CP receives only $1$ request (from $r^1$ only), but both the robots participate. 
\end{example}
}

==> 2023_09_16/7_evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:evaluation}


\shortversion
{
    \input{tables/results_table_v5_short.tex}
}
\longversion
{
    \input{tables/results_table_v5.tex}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation and Experimental Setup}
\label{subsec:implementation_and_experimental_setup}

We implement \FnRobot (Algorithm \ref{algo:robot}) and \FnOnDemCPP (Algorithm \ref{algo:ondemcpp}) in a common ROS \longversion{\cite{key_ros}} package
%\footnote{https://bitbucket.org/DaguMitra/asyn\_cov\_pkg/src/master/} 
and run it in a computer having Intel\textsuperscript{\textregistered} Core\textsuperscript{\texttrademark} i7-4770 CPU @ 3.40 GHz and 16 GB of RAM. 
For experimentation, we consider eight large $2$D grid benchmark workspaces from \cite{DBLP:conf/socs/SternSFK0WLA0KB19} of varying size and obstacle density. 
In each workspace, we \textit{incrementally} deploy $R \in \{128, 256, 512\}$ robots and repeat each experiment $10$ times with different initial deployments of the robots to report their mean in the performance metrics (standard deviations are available in~\cite{DBLP:conf/arxiv/MitraS23}). 

% We consider both TurtleBot (introduced before) and Quadcopter\dm{ (introduced below)} in the experimentation.\st{, where the state of a Quadcopter $s^i_j = (x, y) \in W$ is its location in the workspace. 
% Its set of motion primitives is defined as $M$ = \{$\mathtt{Halt (H)}$, $\mathtt{MoveEast (ME)}$, $\mathtt{MoveNorth (MN)}$, $\mathtt{MoveWest (MW)}$, $\mathtt{MoveSouth (MS)}$\}, where $\mathtt{ME, MN, MW}$, and $\mathtt{MS}$ move it to the immediate \textit{east, north, west}, and \textit{south} cell, respectively. }

% We consider both TurtleBot\longversion{ (introduced before)} and Quadcopter\longversion{ (introduced below)} in the experimentation. 

% \shortversion
% {
% \input{4a_turtlebot}
% }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Robots for evaluation}

We consider both TurtleBot (introduced before) and Quadcopter in the experimentation. 
\input{4b_quadcopter_2d}

% \input{4a_turtlebot}

% We take the path cost as the number of moves the corresponding robot performs, where each move takes $\tau = 1\si{\second}$. 
% %\is{We should mention why it is reasonable by providing the grid size and the velocity of the robot.}
% \dm{This is not an unrealistic assumption because the maximum translational velocity of a TurtleBot2 is $0.65\si{\meter}/\si{\second}$ and of a Quadcopter is $16\si{\meter}/\si{\second}$. 
% So, a TurtleBot2 can traverse a cell of size $0.61\si{\meter}$ in an indoor workspace in $\tau = 1\si{\second}$. 
% Similarly, a Quadcopter can traverse a cell of size $5\si{\meter}$ in an outdoor workspace in $\tau = 1\si{\second}$. 
% We demonstrate this in the real experiments described in Section \ref{subsec:sim_and_real}. 
% }
% \is{Could we add references for the velocities?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Evaluation metrics}

We compare \FnOnDemCPP with \FnGAMRCPP\cite{DBLP:conf/iros/MitraS22} in terms of \textit{the mission time} ($T_m$), which is the sum of \textit{the total computation time} ($T_c$) and \textit{the total path execution time} ($T_p$) while ignoring \textit{the total communication time} between the CP and the robots. 
\textit{Total computation time} ($T_c$) is the sum of the computation times spent on \FnOnDemCPPHor across all horizons. 
\textit{Total path execution time} ($T_p$) can be expressed as $T_p = \Lambda \times \tau$, where $\Lambda$ is \textit{the total horizon length} (i.e., the sum of the horizons lengths). 

In our evaluation, we take the path cost as the number of moves the corresponding robot performs, where each move takes $\tau = 1\si{\second}$. 
This is realistic because the maximum transnational velocity of a TurtleBot2 is $0.65\si{\meter}/\si{\second}$~\cite{key_turtlebot2} and that of a Quadcopter is $\sim$ $16\si{\meter}/\si{\second}$~\cite{dji_drones}. 
Thus, to ensure $\tau = 1\si{\second}$, we can keep the grid cell size for a TurtleBot2 up to $0.65\si{\meter}$, which is sufficient considering its size. 
Similarly, the grid cell size up to $16\si{\meter}$ is sufficient for most practical applications involving Quadcopters. 
% So, a TurtleBot2 can traverse a cell of size $0.65\si{\meter}$ in an indoor workspace in $\tau = 1\si{\second}$. 
% Similarly, a Quadcopter can traverse a cell of size $5\si{\meter}$ in an outdoor workspace in $\tau = 1\si{\second}$. 
We demonstrate this in the real experiments described in Section \ref{subsec:sim_and_real}. 

% We take the path cost as the number of moves the corresponding robot performs, where each move takes $\tau = 1\si{\second}$. 
% %\is{We should mention why it is reasonable by providing the grid size and the velocity of the robot.}
% \dm{This is not an unrealistic assumption because the maximum translational velocity of a TurtleBot2 is $0.65\si{\meter}/\si{\second}$ and of a Quadcopter is $16\si{\meter}/\si{\second}$~\cite{dji_drones}.
% So, a TurtleBot2 can traverse a cell of size $0.61\si{\meter}$ in an indoor workspace in $\tau = 1\si{\second}$. 
% Similarly, a Quadcopter can traverse a cell of size $5\si{\meter}$ in an outdoor workspace in $\tau = 1\si{\second}$. 
% We demonstrate this in the real experiments described in Section \ref{subsec:sim_and_real}.} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results and Analysis}
\label{subsec:results_analysis}


We show the experimental results in Table \ref{tab:experimental_results}, where we list workspaces in increasing order of their obstacle-free cell count $|W_{free}|$ for each type of robot. 
%%For clarity, %of Table \ref{tab:experimental_results}, 
%we do not show any standard deviation, which is available in \cite{DBLP:conf/arxiv/MitraS23}.

\subsubsection{Comparison of Mission time}
The total computation time $T_c$ increases with the number of robots $R$ because more robots become participants in a horizon. 
So, assigning $R^*$ participants to $G^*$ unassigned goals and getting their collision-free paths $\Sigma'$ becomes intensive. 
Notice that $T_c$ also increases with the workspace size, specifically with $|W_{free}|$ as the \textit{state-space} increases. 
Unlike \FnGAMRCPP, where all $R$ robots participate in replanning, \FnOnDemCPP replans with $R^* \leq R$ robots. 
It results in substantially smaller $T_c$ in \FnOnDemCPP compared to \FnGAMRCPP. 
%Hence, $T_c$ is less in \FnOnDemCPP. 
    

Next, the total horizon length $\Lambda$ decreases with $R$ as the deployment of more robots expedites the coverage. 
But, it increases with the workspace size since more $W_{free}$ needs to be covered. 
During replanning, \FnGAMRCPP finds paths for $R$ robots without constraint. 
But, \FnOnDemCPP replans for $R^*$ participants while respecting the constraint $\Sigma_{rem}$ of the non-participants. 
As a result, there is an increase in the participants' collision-free path lengths, increasing individual horizon length $\lambda$ and so $\Lambda$. 
Thus, \FnGAMRCPP yields better $T_p$ compared to \FnOnDemCPP. 
For more insights on $T_p$, please refer to Section \RomanNumeralCaps{5}-B.1 in \cite{DBLP:conf/arxiv/MitraS23}.

In summary, \FnOnDemCPP outperforms \FnGAMRCPP in terms of $T_c$, but 
%On the other hand, \FnOnDemCPP 
underperforms in terms of $T_p$. 
As $R$ or the workspace size increases, the gain of \FnOnDemCPP in terms of $T_c$ surpasses its loss in terms of $T_p$ by a noticeable margin. 
As a result, \FnOnDemCPP outperforms \FnGAMRCPP in terms of the mission time $T_m$.

\shortversion
{
\subsubsection{Implication on Energy Consumption}
Table \ref{tab:experimental_results} also shows the amount of time the robots remain stationary while executing the plan ($T_{Halt}$) and the duration for which the robots move ($T_{non-Halt}$). The total path execution time $T_p$ is the sum of these two components, i.e., $T_p = T_{Halt} + T_{non-Halt}$.
%Out of $T_p$, the robots spend $T_{Halt}$ amount of time executing $\mathtt{Halt}$ moves that get prefixed to their paths for collision avoidance during the time parameterization step in a horizon. 
The ground robots like Turtlebot consume energy only for the $T_{non-Halt}$ duration. As Table~\ref{tab:experimental_results} shows, 
$T_{non-Halt}$ for \FnOnDemCPP is more than that for \FnGAMRCPP. Thus, the energy consumption for the ground robots for \FnOnDemCPP is also proportionately more than that for \FnGAMRCPP.

The situation is quite different for quadcopters. Once the mission starts, the quadcopters either keeps on  hovering (during path computation and while executing the $\mathtt{Halt}$ primitive) or makes translational movement (while executing $\mathtt{non-Halt}$ movements). Thus, a quadcopter keeps on consuming energy throughout the mission. As \FnOnDemCPP reduces the mission time for large number of robots significantly in comparison to \FnGAMRCPP, it also helps in reducing power consumption in the quadcopters during a mission.

Given that reducing the energy consumption during a mission is more crucial for quadcopters than for the ground robots and that \FnOnDemCPP reduces the mission time for both types of robots, \FnOnDemCPP is established to be superior to \FnGAMRCPP as a CP for a large number of robots.



% Out of $T_p$, the robots spend $T_{Halt}$ amount of time executing $\mathtt{Halt}$ moves that get prefixed to their paths for collision avoidance during the time parameterization step in a horizon. 
% Obtained $T_{Halt}$ indicates that though the participants' collision-free path lengths increase in \FnOnDemCPP, those paths contain a substantial number of $\mathtt{Halt}$ moves, which is beneficial from the energy consumption perspective of a ground robot, like a TurtleBot. 
% At first glance, it may look disadvantageous for an aerial robot, like a Quadcopter, as \textit{hovering} consumes more energy, but it is not. 
% A Quadcopter hovers not only for $T_{Halt}$ duration but also for $T_c$ duration, i.e., during planning. 
% It is evident that $T_c + T_{Halt}$ of \FnOnDemCPP is significantly less than that of \FnGAMRCPP. 
% In a horizon of \FnOnDemCPP, the CP assigns the participants to the unassigned goals $W_g \setminus \widetilde{W_g}$ even if some participants can cover some reserved goals $\widetilde{W_g}$ in a more cost-optimal way than their corresponding non-participants. 
% It results in a marginal increase in the number of non-$\mathtt{Halt}$ moves executed and the time $T_{non-Halt}$ spent on it. 
% For more insights on $T_p$, please refer to Section \RomanNumeralCaps{5}-B.1 in \cite{DBLP:conf/arxiv/MitraS23}. 
}

 



\subsubsection{Limitation of OnDemCPP}
The results obtained from the \textit{maze-128-128-2} workspace for $R \in \{128,\ 256\}$ show the limitation of \FnOnDemCPP. 
In a \textit{cluttered} workspace with narrow passageways, the flexibility of \FnGAMRCPP allows it to find a more efficient $\Sigma'$, thereby outmatching \FnOnDemCPP in instances with a smaller $R$. 

\longversion
{
    \input{7b_evaluation_ext.tex}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulations and Real Experiments}
\label{subsec:sim_and_real}


% For validation, we perform Gazebo\longversion{\cite{DBLP:conf/iros/KoenigH04}} simulations with $10$ Quadcopters in five $2$D grid benchmark workspaces from \cite{DBLP:conf/socs/SternSFK0WLA0KB19} and one outdoor experiment with two Quadcopters, whose videos are available as supplementary material. 

For validation, we perform Gazebo\longversion{\cite{DBLP:conf/iros/KoenigH04}} simulations in five $2$D grid benchmark workspaces from \cite{DBLP:conf/socs/SternSFK0WLA0KB19} with $10$ Quadcopters and $10$ TurtleBots, respectively. 
% We also perform one indoor experiment, as shown in Figure \ref{subfig:tb_ws}, with two TurtleBots having initial states $(2, 2, \mathtt{E})$ and $(3, 4, \mathtt{E})$, respectively. 
% Note that the workspace's origin is at the bottom right corner. 
% Each TurtleBot2 is fitted with four HC SR04 Ultrasonic Sound Sensors, as shown in Figures \ref{subfig:tb_f} and \ref{subfig:tb_b}, for obstacle detection, and takes $\tau = 1\si{\second}$ to execute the motion primitives. 
% In addition, we perform one outdoor experiment with two Quadcopters fitted with here$3$ GPS. 
We also perform two real experiments - one indoor with two TurtleBot2s, each fitted with four HC SR$04$ Ultrasonic Sound Sensors for obstacle detection and using Vicon~\cite{key_vicon} for localization, 
%as shown in Figure \ref{subfig:indoor_ws}, 
and one outdoor with three Quadcopters, each fitted with one Cube Orange autopilot, one Herelink Air Unit for communication with the remote controller, and one Here$3$ GPS for localization. 
The workspaces for these experiments are shown in  Figure \ref{subfig:indoor_ws} and Figure \ref{subfig:outdoor_ws}, respectively. 
All these videos are available as supplementary material. 

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.45\linewidth}
%         \centering
%         \includegraphics[scale=0.0285]{figures/tb/5x10_2.png}
%         \caption{$5\times10$ workspace having cell size $0.61\si{\meter}$ and Vicon\cite{key_vicon}}
%         \label{subfig:tb_ws}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.26\linewidth}
%         \centering
%         \includegraphics[scale=0.021]{figures/tb/F.png}
%         \caption{Front view of TurtleBot2}
%         \label{subfig:tb_f}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.26\linewidth}
%         \centering
%         \includegraphics[scale=0.021]{figures/tb/B.png}
%         \caption{Rear view of TurtleBot2}
%         \label{subfig:tb_b}
%     \end{subfigure}
%     \caption{Indoor experiment with two TurtleBots}
%     % \label{fig:tb_real_exp}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        %\includegraphics[scale=0.137]
        \includegraphics[scale=0.025]{figures/tb/5x10_2.pdf}
        \caption{$\phantom{0}5\times10$ indoor workspace [cell size = $0.61\si{\meter}$]}       % ,\ |W_{free}| = 39
        \label{subfig:indoor_ws}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[scale=0.125]{figures/outdoor/outdoor_ws_v2c.pdf}
        \caption{$10\times10$ outdoor workspace [cell size = $5\si{\meter}$]}       % ,\ |W_{free}| = 100
        \label{subfig:outdoor_ws}
    \end{subfigure}
    \caption{Workspaces for the real experiments}
    % \label{fig:}
\end{figure}

% \input{tables/real_exp_short}

==> algorithms/ondemcpp_hor.tex <==
\begin{algorithm}[t!]
    \small
    \DontPrintSemicolon
    
    \caption{}
    \label{algo:ondemcpp_hor}
    
    % \KwResult{}
    \Fn{\FnOnDemCPPHor{}}{
        $\Sigma' \gets \emptyset$       \tcp*{Participants' collision-free paths}
        
        \If{$(W_g\setminus\widetilde{W_g})\neq\emptyset$}{
            $\Sigma' \gets \FnCPPForPar(W, \widetilde{W_g}, I_{par}, S, M, R, \Sigma_{rem})$\;
        }
        \ElseIf{$I_{par} \neq [R]$}{
            \For{$i \in I_{par}$}{
                $\sigma'^i \gets s^i_0$\;
                $\Sigma' \gets \Sigma' \cup \{\sigma'^i\}$
            }
        }
        \Else{
            \Exit()     \tcp*{Coverage Complete !!!}
        }

        $\Sigma'_{all} \gets \mathtt{combine\_paths}(I_{par}, \Sigma', R, \Sigma_{rem})$\;
        $\lambda \gets \mathtt{determine\_horizon\_length}(\Sigma'_{all})$\;
        % $\lambda \gets \min_{i \in [R]}\{|\sigma'^i_{all}|\ |\ |\sigma'^i_{all}| > 0\}$\tcp*{Horizon length}
        $\Sigma \gets$ \FGetEqLenPaths($\Sigma'_{all}, \lambda$)\;
        \Return $\Sigma$\;
    }
    \BlankLine
    \Fn{\FGetEqLenPaths{$\Sigma'_{all}, \lambda$}}{
        $\Sigma \gets \emptyset$, $\Sigma_{rem} \gets \emptyset$, $\widetilde{W_g} \gets \emptyset$, $I^{inact}_{par} \gets \emptyset$, $S^{inact} \gets \emptyset$\;
        $N_{act} \gets 0$       \tcp*{Reinit.}
    
        \For{$i \in [R]$}{
            \If{$|\sigma'^i_{all}| > 0$}{
                $N_{act} \gets N_{act} + 1$     \tcp*{$r^i$ is active}
                $\langle \sigma^i, \sigma^i_{rem} \rangle \gets \mathtt{split\_path}(\sigma'^i_{all}, \lambda)$\;
                $\Sigma \gets \Sigma \cup \{\sigma^i\}$\;

                \If{$|\sigma^i_{rem}| > 0$}{
                    $\widetilde{W_g} \gets \widetilde{W_g} \cup \{\mathcal{L}(s^i_{|\sigma'^i_{all}|})\}$       \tcp*{Reserve}
                }
                \Else{
                    $\sigma^i_{rem} \gets \mathsf{NULL}$\;
                }
                
                $\pi^i \gets \pi^i : \sigma^i$      \tcp*{Concat.}
            }
            \Else{
                $I^{inact}_{par} \gets I^{inact}_{par} \cup \{i\}$      \tcp*{$r^i$ is inactive}
                $S^{inact} \gets S^{inact} \cup \{s^i_0\}$\;
                $\sigma^i_{rem} \gets \mathsf{NULL}$\;
                $\pi^i \gets \pi^i : \mathtt{dummy\_path}(s^i_0, \lambda)$      \tcp*{Concat.}
            }
            
            $\Sigma_{rem} \gets \Sigma_{rem} \cup \{\sigma^i_{rem}\}$\;
        }

        \Return $\Sigma$
    }
\end{algorithm}

==> algorithms/ondemcpp_v3.tex <==
\begin{algorithm}[t!]
    \small
    \DontPrintSemicolon
    
    \caption{$\mathtt{OnDemCPP}(R, X, Y)$}
    \label{algo:ondemcpp}
    
    % \KwResult{}

    $\Sigma_{rem} \gets \{\mathsf{NULL}\ |\ i \in [R]\}$      \tcp*{Init.}
    $I_{par} \gets \emptyset$, $S \gets \emptyset$, $I^{inact}_{par} \gets \emptyset$, $S^{inact} \gets \emptyset$, $W \gets \emptyset$, $\widetilde{W_g} \gets \emptyset$, $\Pi \gets \emptyset$\;
    $N_{req} \gets 0$       \tcp*{Number of requests}
    $N_{act} \gets R$       \tcp*{Number of active robots}    
    \BlankLine
    \Srv{\FRcvLV{$\mathtt{M_{req}}$}}{
        % \tikzmk{A}
        $i \gets \mathtt{M_{req}.id}$       \tcp*{Robot ID}
        
        \If{$\sigma^i_{rem} = \mathsf{NULL}$}{
            $I_{par} \gets I_{par} \cup \{i\}$      \tcp*{$r^i$ is a participant}
            $S \gets S \cup \{\mathtt{M_{req}.state}\}$\;
        }
        
        $\FnUpdateGlobalview(\mathtt{M_{req}.view})$\;
        $N_{req} \gets N_{req} + 1$\;

        \If{$(N_{req} = N_{act})$}{
            $I_{par} \gets I_{par} \cup I^{inact}_{par}$     \tcp*{Formerly inactive}
            $S \gets S \cup S^{inact}$\;
            $\Sigma \gets$ \FnOnDemCPPHor()      \tcp*{Equal-length paths}
            \FnSndPathsToActRobs($\Sigma$)\;
            $I_{par} \gets \emptyset$, $S \gets \emptyset$      \tcp*{Reinit.}
            $N_{req} \gets 0$\;
        }
        % \tikzmk{B}
        % \boxit{lightgray}
    }
    \BlankLine
    \Fn{\FnSndPathsToActRobs{$\Sigma$}}{
        \ParFor{$i \in [R] \setminus I^{inact}_{par}$}{
              \ \ \ \ $\mathtt{M_{res}[path]} \gets \sigma^i$      \tcp*{Create $\mathtt{M_{res}}$}
              \ \ \ \ \ \FSndPath($\mathtt{M_{res}, i}$)\;
        }
    }
\end{algorithm}

==> tables/indoor_exp_results.tex <==
\begin{table}[t]
    \caption{Results of the indoor experiment}
    \label{tab:indoor_exp_results}
    \centering
    \small
    \resizebox{0.99\linewidth}{!}
    {
        \begin{tabular}{ccccccc}
            \toprule

            $R$ & $R^*$ & $T_c\ (\si{\second})$ & $T_p\ (\si{\second})$ & $T_{Halt}\ (\si{\second})$ & $T_{non-Halt}\ (\si{\second})$ & $T_m\ (\si{\second})$ \\

            \midrule

            1 & 1.000 $\pm$ 0.000 & 0.098 $\pm$ 0.001 & 82.500 $\pm$ 1.732 & 0.000 $\pm$ 0.000 & 82.500 $\pm$ 1.732 & 166.026 $\pm$ 3.459 \\
            
            2 & 1.317 $\pm$ 0.080 & 0.141 $\pm$ 0.003 & 46.667 $\pm$ 2.582 & 1.667 $\pm$ 2.066 & 45.000 $\pm$ 1.414 & \phantom{0}95.915 $\pm$ 5.730 \\
            
            % 3 &  &  &  &  &  &  \\
            
            \bottomrule
        \end{tabular}
   }
\end{table}

==> tables/real_exp.tex <==
\begin{table}[t]
    \caption{Results of the real experiments}
    \label{tab:real_exp}
    \centering
    \small
    \resizebox{0.99\linewidth}{!}
    {
        \begin{tabular}{lccccccc}
            \toprule

            $M$ & $R$ & $R^*$ & $T_c\ (\si{\second})$ & $T_p\ (\si{\second})$ & $T_{Halt}\ (\si{\second})$ & $T_{non-Halt}\ (\si{\second})$ & $T_m\ (\si{\second})$ \\

            \midrule

            \multirow{2}{*}{\begin{turn}{90}QC\end{turn}} & 1 & 1.000 $\pm$ 0.000 & 0.205 $\pm$ 0.000 & 99.000 $\pm$ 0.000 & 0.000 $\pm$ 0.000 & 99.000 $\pm$ 0.000 & 203.936 $\pm$ 15.717 \\
            
            & 2 & 1.880 $\pm$ 0.041 & 0.124 $\pm$ 0.000 & 52.667 $\pm$ 1.155 & 0.500 $\pm$ 0.000 & 52.167 $\pm$ 1.155 & 158.354 $\pm$ 6.701 \\
            
            % 3 &  &  &  &  &  &  \\

            \midrule

            \multirow{2}{*}{\begin{turn}{90}TB\end{turn}} & 1 & 1.000 $\pm$ 0.000 & 0.098 $\pm$ 0.001 & 82.500 $\pm$ 1.732 & 0.000 $\pm$ 0.000 & 82.500 $\pm$ 1.732 & 166.026 $\pm$ 3.459 \\
            
            & 2 & 1.317 $\pm$ 0.080 & 0.141 $\pm$ 0.003 & 46.667 $\pm$ 2.582 & 1.667 $\pm$ 2.066 & 45.000 $\pm$ 1.414 & \phantom{0}95.915 $\pm$ 5.730 \\
            
            % 3 &  &  &  &  &  &  \\
            
            \bottomrule
        \end{tabular}
   }
\end{table}

==> tables/real_exp_short.tex <==
\begin{table}[t]
    \caption{Results of the real experiments}
    \label{tab:real_exp}
    \centering
    \small
    \resizebox{0.99\linewidth}{!}
    {
        \begin{tabular}{lccccccc}
            \toprule

            $M$ & $R$ & $R^*$ & $T_c\ (\si{\second})$ & $T_p\ (\si{\second})$ & $T_{Halt}\ (\si{\second})$ & $T_{non-Halt}\ (\si{\second})$ & $T_m\ (\si{\second})$ \\

            \midrule

            \multirow{2}{*}{\begin{turn}{90}QC\end{turn}} & 1 & 1.000 & 0.205 & 99.000 & 0.000 & 99.000 & 203.936 \\
            
            & 2 & 1.880 & 0.124 & 52.667 & 0.500 & 52.167 & 158.354 \\
            
            %& 3 &  &  &  &  &  &  \\

            \midrule

            \multirow{2}{*}{\begin{turn}{90}TB\end{turn}} & 1 & 1.000 & 0.098  & 82.500 & 0.000 & 82.500 & 166.026 \\
            
            & 2 & 1.317 & 0.141 & 46.667 & 1.667 & 45.000 & \phantom{0}95.915 \\
            
            % 3 &  &  &  &  &  &  \\
            
            \bottomrule
        \end{tabular}
   }
\end{table}

==> tables/results_table_v4.tex <==
\begin{table*}[t]
    \caption{Experimental results}
    \label{tab:experimental_results}
    \centering
    \small
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}lccccrrrrrrc@{}}
            \toprule
            
             &  &  &  &  & \multicolumn{2}{c}{$T_c\ (\si{\second})$} & \multicolumn{2}{c}{$T_p\ (\si{\second})$} & \multicolumn{2}{c}{$T_m\ (\si{\second})$} & \textbf{Mission} \\
             
            \cmidrule(lr){6-7}
            \cmidrule(lr){8-9}
            \cmidrule(lr){10-11}
            
            $M$ & \multicolumn{2}{c}{\textit{Workspace}} & $R$ & $R^*$ & \FnGAMRCPP & \FnOnDemCPP & \FnGAMRCPP & \FnOnDemCPP & \FnGAMRCPP & \FnOnDemCPP & \textbf{speed up} \\
            
            \midrule
            
            \multirow{12}{*}{\begin{turn}{90}Quadcopter\end{turn}} & \multirow{3}{*}{\shortstack{W1:\\ w\_woundedcoast\\ $578 \times 642$\ (34,020)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/w_woundedcoast.pdf}} & 128 & \phantom{0}80.4 (62.9 \%) $\pm$ 3.8 & 619.5 $\pm$ \phantom{0}97.9 & 362.2 $\pm$ \phantom{0}58.4 & 696.2 $\pm$ 55.5 & 1042.0 $\pm$ 149.5 & 1315.7 $\pm$ 148.6 & 1404.2 $\pm$ 167.1 & 0.936 \\
             &  &  & 256 & 170.7 (66.7 \%) $\pm$ 5.7 & 1091.3 $\pm$ 255.3 & 521.7 $\pm$ 150.2 & 416.8 $\pm$ 95.0 & 804.2 $\pm$ 250.9 & 1508.1 $\pm$ 345.3 & 1325.9 $\pm$ 383.0 & 1.137 \\
             % &  &  & 384 & 262.5 (68.4 \%) $\pm$ 8.7 & 961.0 $\pm$ 235.1 & 332.5 $\pm$ \phantom{0}91.8 & 311.7 $\pm$ 93.6 & 601.7 $\pm$ 191.2 & 1272.7 $\pm$ 320.7 & 934.2 $\pm$ 239.1 & 1.362 \\
             &  &  & 512 & 361.5 (70.6 \%) $\pm$ 9.7 & 1815.2 $\pm$ 359.4 & 569.1 $\pm$ 168.6 & 231.8 $\pm$ 33.0 & 557.2 $\pm$ 138.9 & 2047.0 $\pm$ 388.0 & 1126.3 $\pm$ 255.4 & 1.817 \\
             
            \cmidrule(lr){2-12}            
            
             & \multirow{3}{*}{\shortstack{W2:\\ Paris\_1\_256\\ $256 \times 256$\ (47,240)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/Paris_1_256.pdf}} & 128 & \phantom{0}81.3 (63.6 \%) $\pm$ 2.6 & 513.5 $\pm$ \phantom{0}38.4 & 270.4 $\pm$ \phantom{0}37.8 & 815.2 $\pm$ 77.4 & 962.6 $\pm$ 100.8 & 1328.7 $\pm$ 109.8 & 1233.0 $\pm$ 118.8 & 1.077 \\
             &  &  & 256 & 157.2 (61.4 \%) $\pm$ 3.7 & 1461.9 $\pm$ 164.0 & 537.2 $\pm$ \phantom{0}79.6 & 508.0 $\pm$ 22.0 & 656.2 $\pm$ \phantom{0}49.4 & 1969.9 $\pm$ 172.2 & 1193.4 $\pm$ 110.8 & 1.650 \\
             % &  &  & 384 & 242.9 (63.3 \%) $\pm$ 8.6 & 1616.7 $\pm$ 184.0 & 460.3 $\pm$ \phantom{0}65.8 & 372.7 $\pm$ 19.9 & 578.8 $\pm$ \phantom{0}23.9 & 1989.4 $\pm$ 191.1 & 1039.1 $\pm$ \phantom{0}75.6 & 1.915 \\
             &  &  & 512 & 335.6 (65.6 \%) $\pm$ 7.0 & 3338.8 $\pm$ 321.9 & 894.0 $\pm$ 113.6 & 301.1 $\pm$ 19.2 & 455.7 $\pm$ \phantom{0}50.1 & 3639.9 $\pm$ 333.6 & 1349.7 $\pm$ 117.1 & 2.696 \\
             
            \cmidrule(lr){2-12}            
            
             & \multirow{3}{*}{\shortstack{W3:\\ Berlin\_1\_256\\ $256 \times 256$\ (47,540)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/Berlin_1_256.pdf}} & 128 & \phantom{0}83.2 (65.1 \%) $\pm$ 2.5 & 489.3 $\pm$ \phantom{0}36.5 & 238.4 $\pm$ \phantom{0}17.2 & 752.7 $\pm$ \phantom{0}32.6 & 898.2 $\pm$ \phantom{0}63.9 & 1242.0 $\pm$ \phantom{0}67.4 & 1136.6 $\pm$ \phantom{0}65.0 & 1.092 \\
             &  &  & 256 & 167.4 (65.4 \%) $\pm$ 12.1 & 1323.9 $\pm$ 154.2 & 515.2 $\pm$ \phantom{0}69.8 & 564.6 $\pm$ 132.5 & 669.6 $\pm$ \phantom{0}48.9 & 1888.5 $\pm$ 234.1 & 1184.8 $\pm$ 103.3 & 1.593 \\
             % &  &  & 384 & 258.7 (67.4 \%) $\pm$ 19.8 & 1605.3 $\pm$ 264.7 & 472.3 $\pm$ \phantom{0}77.5 & 457.2 $\pm$ 177.3 & 602.3 $\pm$ \phantom{0}90.6 & 2062.5 $\pm$ 329.4 & 1074.6 $\pm$ 152.3 & 1.919 \\
             &  &  & 512 & 365.2 (71.3 \%) $\pm$ 34.5 & 3196.5 $\pm$ 329.4 & 856.0 $\pm$ 115.1 & 434.5 $\pm$ 209.9 & 524.9 $\pm$ 140.0 & 3631.0 $\pm$ 434.1 & 1380.9 $\pm$ 238.9 & 2.629 \\
             
            \cmidrule(lr){2-12}            
            
             & \multirow{3}{*}{\shortstack{W4:\\ Boston\_0\_256\\ $256 \times 256$\ (47,768)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/Boston_0_256.pdf}} & 128 & \phantom{0}79.6 (62.2 \%) $\pm$ 4.5 & 509.5 $\pm$ \phantom{0}36.4 & 250.6 $\pm$ \phantom{0}30.1 & 773.6 $\pm$ 61.7 & 928.0 $\pm$ 100.6 & 1283.1 $\pm$ \phantom{0}94.0 & 1178.6 $\pm$ 116.3 & 1.088 \\
             &  &  & 256 & 157.8 (61.7 \%) $\pm$ 9.3 & 1220.1 $\pm$ 215.0 & 455.7 $\pm$ \phantom{0}61.2 & 460.3 $\pm$ 44.8 & 625.9 $\pm$ \phantom{0}46.9 & 1680.4 $\pm$ 256.8 & 1081.6 $\pm$ \phantom{0}92.4 & 1.553 \\
             % &  &  & 384 & 247.1 (64.4 \%) $\pm$ 6.0 & 1319.3 $\pm$ 170.8 & 372.9 $\pm$ \phantom{0}44.4 & 328.9 $\pm$ 18.7 & 547.8 $\pm$ \phantom{0}37.3 & 1648.2 $\pm$ 177.2 & 920.7 $\pm$ \phantom{0}64.6 & 1.790 \\
             &  &  & 512 & 345.3 (67.5 \%) $\pm$ 7.7 & 2454.7 $\pm$ 525.7 & 628.7 $\pm$ 119.3 & 252.9 $\pm$ 23.5 & 428.7 $\pm$ \phantom{0}69.2 & 2707.6 $\pm$ 546.1 & 1057.4 $\pm$ 182.2 & 2.560 \\
             
            \midrule
            
            \multirow{12}{*}{\begin{turn}{90}TurtleBot\end{turn}} & \multirow{3}{*}{\shortstack{W5:\\ maze-128-128-2\\ $128 \times 128$\ (10,858)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/maze-128-128-2.pdf}} & 128 & \phantom{0}75.5 (59.0 \%) $\pm$ 7.4 & 90.8 $\pm$ 19.3 & 49.5 $\pm$ 19.8 & 451.9 $\pm$ 71.7 & 791.5 $\pm$ 202.1 & 542.7 $\pm$ 88.6 & 841.0 $\pm$ 217.7 & 0.645 \\
             &  &  & 256 & 174.7 (68.3 \%) $\pm$ 7.5 & 193.6 $\pm$ 27.1 & 68.1 $\pm$ 16.9 & 218.6 $\pm$ 35.6 & 417.6 $\pm$ \phantom{0}97.4 & 412.2 $\pm$ 58.7 & 485.7 $\pm$ 113.7 & 0.848 \\
             % &  &  & 384 & 273.9 (71.3 \%) $\pm$ 8.7 & 228.5 $\pm$ 26.3 & 56.7 $\pm$ 11.7 & 161.3 $\pm$ 18.8 & 307.8 $\pm$ \phantom{0}31.8 & 389.8 $\pm$ 34.1 & 364.5 $\pm$ \phantom{0}37.1 & 1.070 \\
             &  &  & 512 & 378.4 (73.9 \%) $\pm$ 6.8 & 411.1 $\pm$ 64.7 & 124.1 $\pm$ 23.9 & 125.9 $\pm$ 24.8 & 224.3 $\pm$ \phantom{0}32.1 & 537.0 $\pm$ 71.1 & 348.4 $\pm$ \phantom{0}54.1 & 1.541 \\
             
            \cmidrule(lr){2-12}            
            
             & \multirow{3}{*}{\shortstack{W6:\\ den520d\\ $257 \times 256$\ (28,178)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/den520d.pdf}} & 128 & \phantom{0}71.9 (56.2 \%) $\pm$ 3.2 & 341.8 $\pm$ \phantom{0}50.5 & 147.6 $\pm$ 17.7 & 556.4 $\pm$ 71.4 & 773.1 $\pm$ 106.9 & 898.2 $\pm$ 121.2 & 920.7 $\pm$ 117.7 & 0.975 \\
             &  &  & 256 & 153.8 (60.1 \%) $\pm$ 3.7 & 685.4 $\pm$ 121.5 & 253.9 $\pm$ 63.1 & 324.2 $\pm$ 56.5 & 506.4 $\pm$ \phantom{0}57.4 & 1009.6 $\pm$ 175.2 & 760.3 $\pm$ 103.4 & 1.327 \\
             % &  &  & 384 & 237.1 (61.8 \%) $\pm$ 8.1 & 744.8 $\pm$ 125.6 & 185.6 $\pm$ 27.7 & 241.7 $\pm$ 32.9 & 425.3 $\pm$ \phantom{0}66.5 & 986.5 $\pm$ 145.4 & 610.9 $\pm$ \phantom{0}72.8 & 1.615 \\
             &  &  & 512 & 331.1 (64.7 \%) $\pm$ 6.6 & 1292.4 $\pm$ 304.0 & 316.0 $\pm$ 29.2 & 188.7 $\pm$ \phantom{0}9.2 & 398.6 $\pm$ \phantom{0}37.9 & 1481.1 $\pm$ 301.9 & 714.6 $\pm$ \phantom{0}51.7 & 2.072 \\
             
            \cmidrule(lr){2-12}            
            
             & \multirow{3}{*}{\shortstack{W7:\\ warehouse-20-40-10-2-2\\ $164 \times 340$\ (38,756)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/warehouse-20-40-10-2-2.pdf}} & 128 & \phantom{0}81.2 (63.5 \%) $\pm$ 2.6 & 467.1 $\pm$ \phantom{0}40.0 & 211.3 $\pm$ 22.2 & 595.6 $\pm$ 43.1 & 707.6 $\pm$ \phantom{0}82.5 & 1062.7 $\pm$ \phantom{0}75.2 & 918.9 $\pm$ \phantom{0}98.3 & 1.156 \\
             &  &  & 256 & 149.3 (58.3 \%) $\pm$ 8.1 & 1009.5 $\pm$ 165.2 & 336.0 $\pm$ 31.2 & 361.6 $\pm$ 25.2 & 502.5 $\pm$ \phantom{0}78.2 & 1371.1 $\pm$ 185.3 & 838.5 $\pm$ 100.4 & 1.635 \\
             % &  &  & 384 & 243.0 (63.3 \%) $\pm$ 5.0 & 992.9 $\pm$ 108.7 & 237.4 $\pm$ 30.7 & 269.7 $\pm$ 12.3 & 442.2 $\pm$ \phantom{0}42.8 & 1262.6 $\pm$ 117.9 & 679.6 $\pm$ \phantom{0}72.0 & 1.858 \\
             &  &  & 512 & 335.5 (65.5 \%) $\pm$ 7.2 & 1646.2 $\pm$ 343.7 & 394.7 $\pm$ 36.6 & 208.9 $\pm$ 18.0 & 375.2 $\pm$ \phantom{0}29.5 & 1855.1 $\pm$ 357.5 & 769.9 $\pm$ \phantom{0}54.7 & 2.409 \\
             
            \cmidrule(lr){2-12}            
            
             & \multirow{3}{*}{\shortstack{W8:\\ brc202d\\ $481 \times 530$\ (43,151)}} & \multirow{3}{*}{\includegraphics[scale=0.029]{figures/workspaces/brc202d.pdf}} & 128 & \phantom{0}65.1 (50.9 \%) $\pm$ 3.5 & 1019.0 $\pm$ 160.9 & 395.2 $\pm$ \phantom{0}70.7 & 915.9 $\pm$ 116.4 & 1444.9 $\pm$ 232.0 & 1934.9 $\pm$ 274.3 & 1840.1 $\pm$ 273.6 & 1.051 \\
             &  &  & 256 & 142.0 (55.5 \%) $\pm$ 8.7 & 1880.7 $\pm$ 275.0 & 697.7 $\pm$ 152.3 & 512.5 $\pm$ \phantom{0}60.8 & 972.5 $\pm$ 147.1 & 2393.2 $\pm$ 326.5 & 1670.2 $\pm$ 230.3 & 1.432 \\
             % &  &  & 384 & 223.1 (58.1 \%) $\pm$ 8.1 & 1553.3 $\pm$ 237.8 & 355.2 $\pm$ \phantom{0}56.3 & 372.7 $\pm$ \phantom{0}37.7 & 879.3 $\pm$ 137.3 & 1926.0 $\pm$ 265.2 & 1234.5 $\pm$ 126.7 & 1.560 \\
             &  &  & 512 & 309.6 (60.5 \%) $\pm$ 9.5 & 3026.8 $\pm$ 326.8 & 705.6 $\pm$ 112.5 & 302.6 $\pm$ \phantom{0}21.6 & 780.9 $\pm$ \phantom{0}98.5 & 3329.4 $\pm$ 322.3 & 1486.5 $\pm$ 163.1 & 2.239 \\
            \bottomrule
        \end{tabular}
   }
\vspace{-0.3cm}
\end{table*}

==> tables/results_table_v4_short.tex <==
\begin{table*}[t]
    \caption{Experimental results}
    \label{tab:experimental_results}
    \centering
    \small
    \resizebox{0.99\textwidth}{!}{      % 0.99 -> 0.91
        \begin{tabular}{@{}lccccrrrrrrrrrrc@{}}
            \toprule
            
             &  &  &  &  & \multicolumn{2}{c}{$T_c\ (\si{\second})$} & \multicolumn{2}{c}{$T_p\ (\si{\second})$} & \multicolumn{2}{c}{$T_{Halt}\ (\si{\second})$} & \multicolumn{2}{c}{$T_{non-Halt}\ (\si{\second})$} & \multicolumn{2}{c}{$T_m\ (\si{\second})$} & \textbf{Mission} \\
             
            \cmidrule(lr){6-7}
            \cmidrule(lr){8-9}
            \cmidrule(lr){10-11}
            \cmidrule(lr){12-13}
            \cmidrule(lr){14-15}
            
            $M$ & \multicolumn{2}{c}{\textit{Workspace}} & $R$ & $R^*$ & \FnGAMRCPP & \FnOnDemCPP & \FnGAMRCPP & \FnOnDemCPP & \FnGAMRCPP & \FnOnDemCPP & \FnGAMRCPP & \FnOnDemCPP & \FnGAMRCPP & \FnOnDemCPP & \textbf{speed up} \\
            
            \midrule
            
            \multirow{12}{*}{\begin{turn}{90}Quadcopter\end{turn}} & \multirow{3}{*}{\shortstack{w\_woundedcoast\\  $578 \times 642$\\ (34,020)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/w_woundedcoast.pdf}} & 128 & \phantom{0}80.4 & 619.5 & 362.2 & 696.2 & 1042.0 & 230.8 & 487.4 & 465.4 & 554.5 & 1315.7 & 1404.2 & 0.936 \\
             &  &  & 256 & 170.7 & 1091.3 & 521.7 & 416.8 & 804.2 & 182.3 & 512.2 & 234.5 & 291.9 & 1508.1 & 1325.9 & 1.137 \\
             % &  &  & 384 & 262.5 & 961.0 & 332.5 & 311.7 & 601.7 & 153.5 &	404.3 & 158.2 & 197.3 & 1272.7 & 934.2 & 1.362 \\
             &  &  & 512 & 361.5 & 1815.2 & 569.1 & 231.8 & 557.2 & 115.7 & 404.1 & 116.1 & 153.0 & 2047.0 & 1126.3 & 1.817 \\
             
            \cmidrule(lr){2-16}            
            
             & \multirow{3}{*}{\shortstack{Paris\_1\_256\\ $256 \times 256$\\ (47,240)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/Paris_1_256.pdf}} & 128 & \phantom{0}81.3 & 513.5 & 270.4 & 815.2 & 962.6 & 214.9 & 298.2 & 600.3 & 664.3 & 1328.7 & 1233.0 & 1.077 \\
             &  &  & 256 & 157.2 & 1461.9 & 537.2 & 508.0 & 656.2 & 184.2 & 273.0 & 323.8 & 383.1 & 1969.9 & 1193.4 & 1.650 \\
             % &  &  & 384 & 242.9 & 1616.7 & 460.3 & 372.7 & 578.8 & 154.3 & 300.9 & 218.4 & 277.8 & 1989.4 & 1039.1 & 1.915 \\
             &  &  & 512 & 335.6 & 3338.8 & 894.0 & 301.1 & 455.7 & 137.6 & 247.1 & 163.5 & 208.5 & 3639.9 & 1349.7 & 2.696 \\
             
            \cmidrule(lr){2-16}            
            
             & \multirow{3}{*}{\shortstack{Berlin\_1\_256\\ $256 \times 256$\\ (47,540)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/Berlin_1_256.pdf}} & 128 & \phantom{0}83.2 & 489.3 & 238.4 & 752.7 & 898.2 & 169.9 & 272.9 & 582.8 & 625.2 & 1242.0 & 1136.6 & 1.092 \\
             &  &  & 256 & 167.4 & 1323.9 & 515.2 & 564.6 & 669.6 & 258.0 & 301.0 & 306.6 & 368.5 & 1888.5 & 1184.8 & 1.593 \\
             % &  &  & 384 & 258.7 & 1605.3 & 472.3 & 457.2 & 602.3 & 247.9 &	333.0 & 209.3 & 269.2 & 2062.5 & 1074.6 & 1.919 \\
             &  &  & 512 & 365.2 & 3196.5 & 856.0 & 434.5 & 524.9 & 275.8 & 324.8 & 158.7 & 200.0 & 3631.0 & 1380.9 & 2.629 \\
             
            \cmidrule(lr){2-16}            
            
             & \multirow{3}{*}{\shortstack{Boston\_0\_256\\ $256 \times 256$\\ (47,768)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/Boston_0_256.pdf}} & 128 & \phantom{0}79.6 & 509.5 & 250.6 & 773.6 & 928.0 & 169.4 & 262.6 & 604.2 & 665.3 & 1283.1 & 1178.6 & 1.088 \\
             &  &  & 256 & 157.8 & 1220.1 & 455.7 & 460.3 & 625.9 & 142.5 & 252.0 & 317.8 & 373.8 & 1680.4 & 1081.6 & 1.553 \\
             % &  &  & 384 & 247.1 & 1319.3 & 372.9 & 328.9 & 547.8 & 117.7 & 286.3 & 211.2 & 261.4 & 1648.2 & 920.7 & 1.790 \\
             &  &  & 512 & 345.3 & 2454.7 & 628.7 & 252.9 & 428.7 & 95.6 & 236.7 & 157.3 & 191.9 & 2707.6 & 1057.4 & 2.560 \\
             
            \midrule
            
            \multirow{12}{*}{\begin{turn}{90}TurtleBot\end{turn}} & \multirow{3}{*}{\shortstack{maze-128-128-2\\ $128 \times 128$\\ (10,858)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/maze-128-128-2.pdf}} & 128 & \phantom{0}75.5 & 90.8 & 49.5 & 451.9 & 791.5 & 217.1 & 509.8 & 234.8 & 281.6 & 542.7 & 841.0 & 0.645 \\
             &  &  & 256 & 174.7 & 193.6 & 68.1 & 218.6 & 417.6 & 115.7 &	294.8 & 102.9 & 122.7 & 412.2 & 485.7 & 0.848 \\
             % &  &  & 384 & 273.9 & 228.5 & 56.7 & 161.3 & 307.8 & 96.6 & 225.8 & 64.7 & 81.9 & 389.8 & 364.5 & 1.070 \\
             &  &  & 512 & 378.4 & 411.1 & 124.1 & 125.9 & 224.3 & 79.4 & 165.9 & 46.5 & 58.3 & 537.0 & 348.4 & 1.541 \\
             
            \cmidrule(lr){2-16}            
            
             & \multirow{3}{*}{\shortstack{den520d\\ $257 \times 256$\\ (28,178)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/den520d.pdf}} & 128 & \phantom{0}71.9 & 341.8 & 147.6 & 556.4 & 773.1 & 151.6 & 286.1 & 404.8 & 486.9 & 898.2 & 920.7 & 0.975 \\
             &  &  & 256 & 153.8 & 685.4 & 253.9 & 324.2 & 506.4 & 118.5 & 247.1 & 205.7 & 259.3 & 1009.6 & 760.3 & 1.327 \\
             % &  &  & 384 & 237.1 & 744.8 & 185.6 & 241.7 & 425.3 & 101.4 & 238.6 & 140.3 & 186.6 & 986.5 & 610.9 & 1.615 \\
             &  &  & 512 & 331.1 & 1292.4 & 316.0 & 188.7 & 398.6 & 82.8 & 252.9 & 105.9 & 145.6 & 1481.1 & 714.6 & 2.072 \\
             
            \cmidrule(lr){2-16}            
            
             & \multirow{3}{*}{\shortstack{warehouse-20-40-10-2-2\\ $164 \times 340$\\ (38,756)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/warehouse-20-40-10-2-2.pdf}} & 128 & \phantom{0}81.2 & 467.1 & 211.3 & 595.6 & 707.6 & 115.2 & 187.2 & 480.4 & 520.3 & 1062.7 & 918.9 & 1.156 \\
             &  &  & 256 & 149.3 & 1009.5 & 336.0 & 361.6 & 502.5 & 102.2 & 182.8 & 259.4 & 319.6 & 1371.1 & 838.5 & 1.635 \\
             % &  &  & 384 & 243.0 & 992.9 & 237.4 & 269.7 & 442.2 & 94.2 & 216.8 & 175.5 & 225.3 & 1262.6 & 679.6 & 1.858 \\
             &  &  & 512 & 335.5 & 1646.2 & 394.7 & 208.9 & 375.2 & 75.5 & 204.8 & 133.4 & 170.3 & 1855.1 & 769.9 & 2.409 \\
             
            \cmidrule(lr){2-16}            
            
             & \multirow{3}{*}{\shortstack{brc202d\\ $481 \times 530$\\ (43,151)}} & \multirow{3}{*}{\includegraphics[scale=0.03]{figures/workspaces/brc202d.pdf}} & 128 & \phantom{0}65.1 & 1019.0 & 395.2 & 915.9 & 1444.9 & 242.5 & 587.4 & 673.4 & 857.4 & 1934.9 & 1840.1 & 1.051 \\
             &  &  & 256 & 142.0 & 1880.7 & 697.7 & 512.5 & 972.5 & 177.9 & 510.9 & 334.6 & 461.5 & 2393.2 & 1670.2 & 1.432 \\
             % &  &  & 384 & 223.1 & 1553.3 & 355.2 & 372.7 & 879.3 & 148.0 & 552.0 & 224.7 & 327.2 & 1926.0 & 1234.5 & 1.560 \\
             &  &  & 512 & 309.6 & 3026.8 & 705.6 & 302.6 & 780.9 & 133.9 & 514.6 & 168.7 & 266.2 & 3329.4 & 1486.5 & 2.239 \\
            \bottomrule
        \end{tabular}
   }
\vspace{-0.3cm}
\end{table*}
